c>1 Non-Critical Strings and Large-N Matrix Field Theory

Motivated by a possible relativistic string description of hadrons we use a discretised light-cone quantisation and Lanczos algorithm to investigate the phase structure of phi^3 matrix field theory in the large N limit. In 1+1 dimensions we confirm the existence of Polyakov's non-critical string theory at the boundary between parton-like and string-like phases, finding critical exponents for longitudinal oscillations equal to or consistent with those given by a mean field argument. The excitation spectrum is finite, possibly discrete. We calculate light-cone structure functions and find evidence that the probability Q(x) of a parton in the string carrying longitudinal momentum fraction between x and x+dx has support on all 0<x<1, despite the average number of partons being infinite.

==> fig2a <==
%!
%%Creator: Mathematica
%%AspectRatio: .61803 
MathPictureStart
%% Graphics
/Courier findfont 10  scalefont  setfont
% Scaling calculations
0 0.0769231 0 0.882906 [
[(1)] .07692 0 0 2 Msboxa
[(2)] .15385 0 0 2 Msboxa
[(3)] .23077 0 0 2 Msboxa
[(4)] .30769 0 0 2 Msboxa
[(5)] .38462 0 0 2 Msboxa
[(6)] .46154 0 0 2 Msboxa
[(7)] .53846 0 0 2 Msboxa
[(8)] .61538 0 0 2 Msboxa
[(9)] .69231 0 0 2 Msboxa
[(10)] .76923 0 0 2 Msboxa
[(11)] .84615 0 0 2 Msboxa
[(12)] .92308 0 0 2 Msboxa
[(n)] 1.025 0 -1 0 Msboxa
[(Fig.2. - \(a\))] .5 .61803 0 -2 0 0 1 Mouter Mrotsboxa
[(0)] -0.0125 0 1 0 Msboxa
[(0.1)] -0.0125 .08829 1 0 Msboxa
[(0.2)] -0.0125 .17658 1 0 Msboxa
[(0.3)] -0.0125 .26487 1 0 Msboxa
[(0.4)] -0.0125 .35316 1 0 Msboxa
[(0.5)] -0.0125 .44145 1 0 Msboxa
[(0.6)] -0.0125 .52974 1 0 Msboxa
[(P\(n\))] 0 .61803 0 -4 Msboxa
[ -0.001 -0.001 0 0 ]
[ 1.001 .61903 0 0 ]
] MathScale
% Start of Graphics
1 setlinecap
1 setlinejoin
newpath
[ ] 0 setdash
0 g
p
p
.002 w
.07692 0 m
.07692 .00625 L
s
P
[(1)] .07692 0 0 2 Mshowa
p
.002 w
.15385 0 m
.15385 .00625 L
s
P
[(2)] .15385 0 0 2 Mshowa
p
.002 w
.23077 0 m
.23077 .00625 L
s
P
[(3)] .23077 0 0 2 Mshowa
p
.002 w
.30769 0 m
.30769 .00625 L
s
P
[(4)] .30769 0 0 2 Mshowa
p
.002 w
.38462 0 m
.38462 .00625 L
s
P
[(5)] .38462 0 0 2 Mshowa
p
.002 w
.46154 0 m
.46154 .00625 L
s
P
[(6)] .46154 0 0 2 Mshowa
p
.002 w
.53846 0 m
.53846 .00625 L
s
P
[(7)] .53846 0 0 2 Mshowa
p
.002 w
.61538 0 m
.61538 .00625 L
s
P
[(8)] .61538 0 0 2 Mshowa
p
.002 w
.69231 0 m
.69231 .00625 L
s
P
[(9)] .69231 0 0 2 Mshowa
p
.002 w
.76923 0 m
.76923 .00625 L
s
P
[(10)] .76923 0 0 2 Mshowa
p
.002 w
.84615 0 m
.84615 .00625 L
s
P
[(11)] .84615 0 0 2 Mshowa
p
.002 w
.92308 0 m
.92308 .00625 L
s
P
[(12)] .92308 0 0 2 Mshowa
[(n)] 1.025 0 -1 0 Mshowa
p
.002 w
0 0 m
1 0 L
s
P
[(Fig.2. - \(a\))] .5 .61803 0 -2 0 0 1 Mouter Mrotshowa
p
.002 w
0 0 m
.00625 0 L
s
P
[(0)] -0.0125 0 1 0 Mshowa
p
.002 w
0 .08829 m
.00625 .08829 L
s
P
[(0.1)] -0.0125 .08829 1 0 Mshowa
p
.002 w
0 .17658 m
.00625 .17658 L
s
P
[(0.2)] -0.0125 .17658 1 0 Mshowa
p
.002 w
0 .26487 m
.00625 .26487 L
s
P
[(0.3)] -0.0125 .26487 1 0 Mshowa
p
.002 w
0 .35316 m
.00625 .35316 L
s
P
[(0.4)] -0.0125 .35316 1 0 Mshowa
p
.002 w
0 .44145 m
.00625 .44145 L
s
P
[(0.5)] -0.0125 .44145 1 0 Mshowa
p
.002 w
0 .52974 m
.00625 .52974 L
s
P
[(0.6)] -0.0125 .52974 1 0 Mshowa
p
.001 w
0 .01766 m
.00375 .01766 L
s
P
p
.001 w
0 .03532 m
.00375 .03532 L
s
P
p
.001 w
0 .05297 m
.00375 .05297 L
s
P
p
.001 w
0 .07063 m
.00375 .07063 L
s
P
p
.001 w
0 .10595 m
.00375 .10595 L
s
P
p
.001 w
0 .12361 m
.00375 .12361 L
s
P
p
.001 w
0 .14126 m
.00375 .14126 L
s
P
p
.001 w
0 .15892 m
.00375 .15892 L
s
P
p
.001 w
0 .19424 m
.00375 .19424 L
s
P
p
.001 w
0 .2119 m
.00375 .2119 L
s
P
p
.001 w
0 .22956 m
.00375 .22956 L
s
P
p
.001 w
0 .24721 m
.00375 .24721 L
s
P
p
.001 w
0 .28253 m
.00375 .28253 L
s
P
p
.001 w
0 .30019 m
.00375 .30019 L
s
P
p
.001 w
0 .31785 m
.00375 .31785 L
s
P
p
.001 w
0 .3355 m
.00375 .3355 L
s
P
p
.001 w
0 .37082 m
.00375 .37082 L
s
P
p
.001 w
0 .38848 m
.00375 .38848 L
s
P
p
.001 w
0 .40614 m
.00375 .40614 L
s
P
p
.001 w
0 .42379 m
.00375 .42379 L
s
P
p
.001 w
0 .45911 m
.00375 .45911 L
s
P
p
.001 w
0 .47677 m
.00375 .47677 L
s
P
p
.001 w
0 .49443 m
.00375 .49443 L
s
P
p
.001 w
0 .51209 m
.00375 .51209 L
s
P
p
.001 w
0 .5474 m
.00375 .5474 L
s
P
p
.001 w
0 .56506 m
.00375 .56506 L
s
P
p
.001 w
0 .58272 m
.00375 .58272 L
s
P
p
.001 w
0 .60038 m
.00375 .60038 L
s
P
[(P\(n\))] 0 .61803 0 -4 Mshowa
p
.002 w
0 0 m
0 .61803 L
s
P
P
0 0 m
1 0 L
1 .61803 L
0 .61803 L
closepath
clip
newpath
p
p
.004 w
.07692 .55599 m
matrix currentmatrix
.00538 .0053 scale
14.2851 104.955 1 0 365.73 arc
setmatrix
F
.15385 .2382 m
matrix currentmatrix
.00538 .0053 scale
28.5721 44.9652 1 0 365.73 arc
setmatrix
F
.23077 .06973 m
matrix currentmatrix
.00538 .0053 scale
42.8573 13.163 1 0 365.73 arc
setmatrix
F
.30769 .01579 m
matrix currentmatrix
.00538 .0053 scale
57.1424 2.98069 1 0 365.73 arc
setmatrix
F
.38462 .00276 m
matrix currentmatrix
.00538 .0053 scale
71.4294 .52101 1 0 365.73 arc
setmatrix
F
.46154 .00038 m
matrix currentmatrix
.00538 .0053 scale
85.7146 .07173 1 0 365.73 arc
setmatrix
F
.53846 0 m
matrix currentmatrix
.00538 .0053 scale
99.9997 0 1 0 365.73 arc
setmatrix
F
.61538 0 m
matrix currentmatrix
.00538 .0053 scale
114.285 0 1 0 365.73 arc
setmatrix
F
.69231 0 m
matrix currentmatrix
.00538 .0053 scale
128.572 0 1 0 365.73 arc
setmatrix
F
.76923 0 m
matrix currentmatrix
.00538 .0053 scale
142.857 0 1 0 365.73 arc
setmatrix
F
.84615 0 m
matrix currentmatrix
.00538 .0053 scale
157.142 0 1 0 365.73 arc
setmatrix
F
.92308 0 m
matrix currentmatrix
.00538 .0053 scale
171.429 0 1 0 365.73 arc
setmatrix
F
P
p
.004 w
newpath
matrix currentmatrix
.00538 .0053 scale
14.2851 .32657 1 0 365.73 arc
setmatrix
s
newpath
matrix currentmatrix
.00538 .0053 scale
28.5721 6.45029 1 0 365.73 arc
setmatrix
s
newpath
matrix currentmatrix
.00538 .0053 scale
42.8573 26.0994 1 0 365.73 arc
setmatrix
s
newpath
matrix currentmatrix
.00538 .0053 scale
57.1424 45.1992 1 0 365.73 arc
setmatrix
s
newpath
matrix currentmatrix
.00538 .0053 scale
71.4294 44.3913 1 0 365.73 arc
setmatrix
s
newpath
matrix currentmatrix
.00538 .0053 scale
85.7146 27.9456 1 0 365.73 arc
setmatrix
s
newpath
matrix currentmatrix
.00538 .0053 scale
99.9997 11.9209 1 0 365.73 arc
setmatrix
s
newpath
matrix currentmatrix
.00538 .0053 scale
114.285 3.49981 1 0 365.73 arc
setmatrix
s
newpath
matrix currentmatrix
.00538 .0053 scale
128.572 .70034 1 0 365.73 arc
setmatrix
s
newpath
matrix currentmatrix
.00538 .0053 scale
142.857 .09627 1 0 365.73 arc
setmatrix
s
newpath
matrix currentmatrix
.00538 .0053 scale
157.142 .00755 1 0 365.73 arc
setmatrix
s
newpath
matrix currentmatrix
.00538 .0053 scale
171.429 0 1 0 365.73 arc
setmatrix
s
P
P
% End of Graphics
MathPictureEnd


==> fig2b <==
%!
%%Creator: Mathematica
%%AspectRatio: .61803 
MathPictureStart
%% Graphics
/Courier findfont 10  scalefont  setfont
% Scaling calculations
0 0.0769231 0 0.0772542 [
[(0.5)] .46154 0 0 2 Msboxa
[(1)] .92308 0 0 2 Msboxa
[(x)] 1.025 0 -1 0 Msboxa
[(Fig.2. - \(b\))] .5 .61803 0 -2 0 0 1 Mouter Mrotsboxa
[(0)] -0.0125 0 1 0 Msboxa
[(1)] -0.0125 .07725 1 0 Msboxa
[(2)] -0.0125 .15451 1 0 Msboxa
[(3)] -0.0125 .23176 1 0 Msboxa
[(4)] -0.0125 .30902 1 0 Msboxa
[(5)] -0.0125 .38627 1 0 Msboxa
[(6)] -0.0125 .46353 1 0 Msboxa
[(7)] -0.0125 .54078 1 0 Msboxa
[(8)] -0.0125 .61803 1 0 Msboxa
[(Q\(x\))] 0 .61803 0 -4 Msboxa
[ -0.001 -0.001 0 0 ]
[ 1.001 .61903 0 0 ]
] MathScale
% Start of Graphics
1 setlinecap
1 setlinejoin
newpath
[ ] 0 setdash
0 g
p
p
.002 w
.46154 0 m
.46154 .00625 L
s
P
[(0.5)] .46154 0 0 2 Mshowa
p
.002 w
.92308 0 m
.92308 .00625 L
s
P
[(1)] .92308 0 0 2 Mshowa
[(x)] 1.025 0 -1 0 Mshowa
p
.002 w
0 0 m
1 0 L
s
P
[(Fig.2. - \(b\))] .5 .61803 0 -2 0 0 1 Mouter Mrotshowa
p
.002 w
0 0 m
.00625 0 L
s
P
[(0)] -0.0125 0 1 0 Mshowa
p
.002 w
0 .07725 m
.00625 .07725 L
s
P
[(1)] -0.0125 .07725 1 0 Mshowa
p
.002 w
0 .15451 m
.00625 .15451 L
s
P
[(2)] -0.0125 .15451 1 0 Mshowa
p
.002 w
0 .23176 m
.00625 .23176 L
s
P
[(3)] -0.0125 .23176 1 0 Mshowa
p
.002 w
0 .30902 m
.00625 .30902 L
s
P
[(4)] -0.0125 .30902 1 0 Mshowa
p
.002 w
0 .38627 m
.00625 .38627 L
s
P
[(5)] -0.0125 .38627 1 0 Mshowa
p
.002 w
0 .46353 m
.00625 .46353 L
s
P
[(6)] -0.0125 .46353 1 0 Mshowa
p
.002 w
0 .54078 m
.00625 .54078 L
s
P
[(7)] -0.0125 .54078 1 0 Mshowa
p
.002 w
0 .61803 m
.00625 .61803 L
s
P
[(8)] -0.0125 .61803 1 0 Mshowa
p
.001 w
0 .01545 m
.00375 .01545 L
s
P
p
.001 w
0 .0309 m
.00375 .0309 L
s
P
p
.001 w
0 .04635 m
.00375 .04635 L
s
P
p
.001 w
0 .0618 m
.00375 .0618 L
s
P
p
.001 w
0 .09271 m
.00375 .09271 L
s
P
p
.001 w
0 .10816 m
.00375 .10816 L
s
P
p
.001 w
0 .12361 m
.00375 .12361 L
s
P
p
.001 w
0 .13906 m
.00375 .13906 L
s
P
p
.001 w
0 .16996 m
.00375 .16996 L
s
P
p
.001 w
0 .18541 m
.00375 .18541 L
s
P
p
.001 w
0 .20086 m
.00375 .20086 L
s
P
p
.001 w
0 .21631 m
.00375 .21631 L
s
P
p
.001 w
0 .24721 m
.00375 .24721 L
s
P
p
.001 w
0 .26266 m
.00375 .26266 L
s
P
p
.001 w
0 .27812 m
.00375 .27812 L
s
P
p
.001 w
0 .29357 m
.00375 .29357 L
s
P
p
.001 w
0 .32447 m
.00375 .32447 L
s
P
p
.001 w
0 .33992 m
.00375 .33992 L
s
P
p
.001 w
0 .35537 m
.00375 .35537 L
s
P
p
.001 w
0 .37082 m
.00375 .37082 L
s
P
p
.001 w
0 .40172 m
.00375 .40172 L
s
P
p
.001 w
0 .41717 m
.00375 .41717 L
s
P
p
.001 w
0 .43262 m
.00375 .43262 L
s
P
p
.001 w
0 .44807 m
.00375 .44807 L
s
P
p
.001 w
0 .47898 m
.00375 .47898 L
s
P
p
.001 w
0 .49443 m
.00375 .49443 L
s
P
p
.001 w
0 .50988 m
.00375 .50988 L
s
P
p
.001 w
0 .52533 m
.00375 .52533 L
s
P
p
.001 w
0 .55623 m
.00375 .55623 L
s
P
p
.001 w
0 .57168 m
.00375 .57168 L
s
P
p
.001 w
0 .58713 m
.00375 .58713 L
s
P
p
.001 w
0 .60258 m
.00375 .60258 L
s
P
[(Q\(x\))] 0 .61803 0 -4 Mshowa
p
.002 w
0 0 m
0 .61803 L
s
P
P
0 0 m
1 0 L
1 .61803 L
0 .61803 L
closepath
clip
newpath
p
p
.004 w
.07692 .01483 m
matrix currentmatrix
.00538 .00541 scale
14.2851 2.74234 1 0 365.73 arc
setmatrix
F
.15385 .02874 m
matrix currentmatrix
.00538 .00541 scale
28.5721 5.31455 1 0 365.73 arc
setmatrix
F
.23077 .04023 m
matrix currentmatrix
.00538 .00541 scale
42.8573 7.43926 1 0 365.73 arc
setmatrix
F
.30769 .04719 m
matrix currentmatrix
.00538 .00541 scale
57.1424 8.72629 1 0 365.73 arc
setmatrix
F
.38462 .04932 m
matrix currentmatrix
.00538 .00541 scale
71.4294 9.12016 1 0 365.73 arc
setmatrix
F
.46154 .04747 m
matrix currentmatrix
.00538 .00541 scale
85.7146 8.77807 1 0 365.73 arc
setmatrix
F
.53846 .04246 m
matrix currentmatrix
.00538 .00541 scale
99.9997 7.85163 1 0 365.73 arc
setmatrix
F
.61538 .0343 m
matrix currentmatrix
.00538 .00541 scale
114.285 6.34269 1 0 365.73 arc
setmatrix
F
.69231 .02341 m
matrix currentmatrix
.00538 .00541 scale
128.572 4.32893 1 0 365.73 arc
setmatrix
F
.76923 .01176 m
matrix currentmatrix
.00538 .00541 scale
142.857 2.17464 1 0 365.73 arc
setmatrix
F
.84615 .00334 m
matrix currentmatrix
.00538 .00541 scale
157.142 .61763 1 0 365.73 arc
setmatrix
F
.92308 .58379 m
matrix currentmatrix
.00538 .00541 scale
171.429 107.953 1 0 365.73 arc
setmatrix
F
P
p
.004 w
newpath
matrix currentmatrix
.00538 .00541 scale
14.2851 38.058 1 0 365.73 arc
setmatrix
s
newpath
matrix currentmatrix
.00538 .00541 scale
28.5721 48.8572 1 0 365.73 arc
setmatrix
s
newpath
matrix currentmatrix
.00538 .00541 scale
42.8573 36.6859 1 0 365.73 arc
setmatrix
s
newpath
matrix currentmatrix
.00538 .00541 scale
57.1424 22.732 1 0 365.73 arc
setmatrix
s
newpath
matrix currentmatrix
.00538 .00541 scale
71.4294 12.6687 1 0 365.73 arc
setmatrix
s
newpath
matrix currentmatrix
.00538 .00541 scale
85.7146 6.53131 1 0 365.73 arc
setmatrix
s
newpath
matrix currentmatrix
.00538 .00541 scale
99.9997 3.16765 1 0 365.73 arc
setmatrix
s
newpath
matrix currentmatrix
.00538 .00541 scale
114.285 1.44976 1 0 365.73 arc
setmatrix
s
newpath
matrix currentmatrix
.00538 .00541 scale
128.572 .61578 1 0 365.73 arc
setmatrix
s
newpath
matrix currentmatrix
.00538 .00541 scale
142.857 .22745 1 0 365.73 arc
setmatrix
s
newpath
matrix currentmatrix
.00538 .00541 scale
157.142 .02219 1 0 365.73 arc
setmatrix
s
newpath
matrix currentmatrix
.00538 .00541 scale
171.429 1.44051 1 0 365.73 arc
setmatrix
s
P
P
% End of Graphics
MathPictureEnd

